ForensiBlock: A Provenance-Driven Blockchain Framework for Data Forensics and Auditability

Maintaining accurate provenance records is paramount in digital forensics, as they underpin evidence credibility and integrity, addressing essential aspects like accountability and reproducibility. Blockchains have several properties that can address these requirements. Previous systems utilized public blockchains, i.e., treated blockchain as a black box, and benefiting from the immutability property. However, the blockchain was accessible to everyone, giving rise to security concerns and moreover, efficient extraction of provenance faces challenges due to the enormous scale and complexity of digital data. This necessitates a tailored blockchain design for digital forensics. Our solution, Forensiblock has a novel design that automates investigation steps, ensures secure data access, traces data origins, preserves records, and expedites provenance extraction. Forensiblock incorporates Role-Based Access Control with Staged Authorization (RBAC-SA) and a distributed Merkle root for case tracking. These features support authorized resource access with an efficient retrieval of provenance records. Particularly, comparing two methods for extracting provenance records off chain storage retrieval with Merkle root verification and a brute-force search the offchain method is significantly better, especially as the blockchain size and number of cases increase. We also found that our distributed Merkle root creation slightly increases smart contract processing time but significantly improves history access. Overall, we show that Forensiblock offers secure, efficient, and reliable handling of digital forensic data

==> Queries.tex <==
\section{Provenance Records}
For preserving the provenance records, tacking the possible malicious modification and verifying them, we incorporate different strategies which involve using both the blockchain and off-chain storage.
%\subsection{Rooted Tree with Directed Acyclic Graph (DAG) Branches}In order to maintain the provenance records for each specific case, we propose the use of a rooted tree structure with directed acyclic graph (DAG) branches. This structure provides an effective means of organizing and tracking the relevant information.The structure is a directed graph G = (V, E), where V represents the set of nodes and E represents the set of directed edges.Each case is identified by a unique case number, denoted as $c \in V$. The case number serves as the root node of the tree.
%The second layer of nodes consists of initial tokens associated with the case. We denote the set of initial tokens as $T_0$, where $t_0 \in T_0$ represents an initial token. Each initial token is connected to the case number node with directed edges, denoted as $(c, t_0) \in E$.
%From the third layer onwards, the structure transitions into a DAG, allowing for derived tokens to be generated. We denote the set of derived tokens as $T$, where $t \in T$ represents a derived token. Each derived token can be connected to one or more parent tokens, and each parent token can have multiple child tokens. Thus, for each derived token $t$ and its parent tokens $p_1, p_2, ..., p_n$, we have directed edges $(p_1, t), (p_2, t), ..., (p_n, t) \in E$.





\subsection{Tokens for Versioning of files for Provenance Tracking}
The relationship among our data exhibits complexity, as illustrated in Figure \ref{fig:dep}. The analyzed data can either be independent or dependent on one another. For instance, files A and B were combined to create file AB, while files B and C were utilized to generate file BC2. Subsequently, files A and BC2 were employed to produce ABC2.

To effectively monitor the versioning and connections between files and have distinct tokens per each file, we propose an algorithm for generating tokens. These tokens act as unique identifiers for file versions and facilitate the creation of a Merkle DAG for each scenario.

\begin{enumerate}
    \item Whenever a new file is created or modified, generate a token for that file to represent its version. Let $K_i$ denote the token for file $i$.
    
    \item To create the derived token for a file, hash the tokens of the initial files from which the derived file is generated. This ensures that the derived file's token is based on the tokens of its parent files. Let $K_{\text{derived}}$ represent the derived token for a file derived from initial files with tokens $K_{\text{initial}_1}, K_{\text{initial}_2}, \ldots, K_{\text{initial}_n}$. The derived token can be computed as:
    
    \[K_{\text{derived}} = \text{hash}(K_{\text{initial}_1}, K_{\text{initial}_2}, \ldots, K_{\text{initial}_n}, \text{Time})\]
    
    where \text{Time} represents the timestamp of the corresponding transaction. Including time in the hash calculation ensures that even if the same files are combined multiple times, different derived tokens will be generated based on the distinct timestamps.
    
  %  \item Add the derived token $K_{\text{derived}}$ as a new node in the Merkle DAG. This node represents the derived file and its relationship to the initial files.
    
  %  \item Establish the relationship between the initial tokens and the derived token by adding an edge in the Merkle DAG. This edge connects the initial tokens to the derived token and signifies the dependency and versioning relationship between the files.
\end{enumerate}

By applying this algorithm, each case will have its own DAG that captures the versioning steps and relationships of the files associated with that case. 
%The Merkle DAG provides an organized and efficient means of tracking the provenance and version history of files within the blockchain. The tree will be stored at the off-blockchain storage.
%The integrity and consistency of files at each version can be verified using the Merkle DAG, as any change in a file will impact the hash values and the Merkle root of the DAG. This ensures secure and reliable provenance tracking within the blockchain system.
\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.6\textwidth]{Sections/Figures/data-dep.jpg}
  \caption{File dependency example per case}
  \label{fig:dep}
\end{figure}


\subsection{Enhancing Provenance Queries}
%One of the unique features of the blockchain design is its ability to streamline data lineage retrieval, thereby enhancing the efficiency of provenance queries. Provenance, which encompasses tracing the origin, ownership, and history of data or digital assets, plays a critical role in establishing data integrity and accountability. In the context of this blockchain design, provenance queries enable users to effortlessly access comprehensive information about a specific case, including its associated edits and historical records.

%To achieve seamless and efficient provenance queries, the design incorporates several key elements. Firstly, each case is assigned an initial block number during the initial request, allowing for easy identification and localization of the case within the blockchain's blocks. Moreover, every transaction within the blockchain is associated with a unique case number, facilitating the extraction of relevant transactions specifically linked to the desired case.

%Additionally, the design employs tokens, which serve as unique identifiers for each file of the case and are stored in the smart contract of every case. These token identifiers are included in the transactions recorded in the blockchain, establishing a seamless link between the data and the tokens. This mechanism simplifies the traversal of the blockchain and enables the construction of a hierarchical representation, resembling a tree-like structure, that effectively captures the sequence of edits made to the data over time.

%By incorporating block numbers, case numbers, and token identifiers, the blockchain design optimizes the process of retrieving data lineage. Users can effortlessly navigate the blockchain, track the origin and history of specific cases, and gain a comprehensive understanding of the data's evolution.




%Compared to alternative methods such as storing the history of edits in storage or versioning, this blockchain-based approach requires less storage space and reduces the need for trust between the parties involved. Moreover, extracting the edit history tree through forward tracking is less complex compared to backward tracking methods. This streamlined approach to provenance queries enhances data transparency, accountability, and trustworthiness within the blockchain ecosystem.
To enhance the extraction of provenance records, two methods are utilized. The first method involves storing the provenance records on the blockchain, which ensures their trustworthiness. The blockchain maintains additional information, such as the unique case number associated with each transaction. This facilitates the extraction of relevant transactions specifically linked to the desired case. The design incorporates tokens as unique identifiers for each file within a case, and these tokens are stored in the smart contract of every case. The transactions recorded in the blockchain include these token identifiers, establishing a seamless link between the data and the tokens. This mechanism simplifies the traversal of the blockchain and enables the construction of a hierarchical representation, resembling a tree-like structure, that effectively captures the sequence of edits made to the data over time. The immutable and trustworthy nature of the blockchain ensures the reliability of the extracted provenance records.

The second method involves storing the records in an off-chain storage system, which allows for faster retrieval of information per case. However, when extracting records from the storage, it is important to verify their trustworthiness. To address this,  we propose that distributed Merkle root for case tracking.

To verify the provenance versioning extracted from the off-chain storage, the block headers in the blockchain contain multiple Merkle roots. Each case added in the block transactions has its own Merkle root, denoted as $M_{\text{case}}$. As shown in Figure\ref{fig:case} This Merkle root is calculated as the hash value of the previous Merkle root associated with the case number, hashed with the transactions added in the current block.

Let $M_{\text{prev\_case}}$ denote the previous Merkle root associated with the case number, and let $T_{\text{block}}$ represent the set of transactions added in the current block. The Merkle root for each case, denoted as $M_{\text{case}}$, is calculated as the hash value of the concatenation of $M_{\text{prev\_case}}$ and $T_{\text{block}}$:

\[ M_{\text{case}} = \text{hash}(M_{\text{prev\_case}} \parallel T_{\text{block}}) \]

This formula ensures that each case added in the block transactions has its own unique Merkle root. By hashing the previous Merkle root with the transactions in the current block, we create a tamper-evident structure that links the provenance records of individual cases from one block to the next.

The utilization of these two methods, storing provenance records on the blockchain and employing distributed Merkle roots, enhances the extraction and verification of provenance records in the system.
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{Sections/Figures/block.jpg}
  \caption{Merkle Root for Distributed Case Tracking}
  \label{fig:case}
\end{figure}


\subsection{Verification of Provenance records}

To ensure the integrity of storage provenance records per case, the verification process outlined in Algorithm \ref{algo:storage_verification} is employed. This algorithm constructs a Merkle tree, depicted in Figure \ref{fig:Merkle-Tree}, and compares the resulting Merkle root with the stored Merkle root. By performing this comparison, it is determined whether any modifications have occurred in the data.


\begin{algorithm}[H]
    \caption{Enhanced Storage Verification}
    \label{algo:storage_verification}
    \begin{algorithmic}[1]
        \Function{EnhancedStorageVerification}{$investigation\_code$}
            \State $selected\_records \gets$ filter $data$ based on $investigation\_code$
            \State $sorted\_records \gets$ sort $selected\_records$ by ascending block number
            
            \State $merkle\_root \gets$ null
            \State $block\_transaction\_strings \gets$ empty list
            
            \For{$record$ \textbf{in} $sorted\_records$}
                \If{$record$ is in a new block}
                    \State $previous\_merkle\_root \gets merkle\_root$
                    \State Compute the Merkle root for the previous block and update $merkle\_root$ using $previous\_merkle\_root$
                    \State $block\_transaction\_strings \gets$ empty list
                \EndIf
                
                \State $serialized\_record \gets$ \Call{SerializeRecord}{$record$}
                \State Append $serialized\_record$ to $block\_transaction\_strings$
            \EndFor
            
            \State $last\_block\_merkle\_root \gets$ Compute the Merkle root for the last block
            \State $merkle\_root \gets$ Update $merkle\_root$ using $last\_block\_merkle\_root$
            
            \State $stored\_merkle\_root \gets$ Retrieve the stored Merkle root for the investigation
            
            \If{$merkle\_root$ matches $stored\_merkle\_root$}
                \State All records are successfully verified for integrity
            \Else
                \State Data integrity has been compromised
            \EndIf
            
            \State \Return $selected\_records$
        \EndFunction
    \end{algorithmic}
\end{algorithm}


%\subsection{Merkle-based Provenance Verification}
%To verify the provenance versioning extracted from the storage, the block headers contain multiple Merkle roots. 

%\begin{enumerate}
  %  \item The first Merkle root, denoted as $M_1$, represents the state-of-the-art Merkle root that verifies all the transactions in the block. It ensures the integrity and consistency of the entire block.
    
   % \item %Each case added in the block transactions has its own Merkle root, denoted as $M_{\text{case}}$. This Merkle root is calculated as the hash value of the previous Merkle root associated with the case number, hashed with the transactions added in the current block as shown in Figure \label{Block}
   % Let $M_{\text{prev\_case}}$ denote the previous Merkle root associated with the case number, and let $T_{\text{block}}$ represent the set of transactions added in the current block.

%The Merkle root for each case, denoted as $M_{\text{case}}$, is calculated as the hash value of the concatenation of $M_{\text{prev\_case}}$ and $T_{\text{block}}$:

%\[ M_{\text{case}} = \text{hash}(M_{\text{prev\_case}} \parallel T_{\text{block}}) \]

%This formula ensures that each case added in the block transactions has its own unique Merkle root. By hashing the previous Merkle root with the transactions in the current block, we create a tamper-evident structure that links the provenance records of individual cases from one block to the next.

    
    %This ensures that each case number can be verified separately and provides a tamper-evident structure for the provenance records of individual cases.
    
   % \item %The derived token, which is created based on the transactions in this block, is added as an additional Merkle root, denoted as $M_{\text{derived}}$. The derived token represents the hash value of the set of tokens related to the transactions in the block. It serves as a reference point for verifying the integrity of the derived token and its relationship with the underlying transactions.
   % To ensure data dependency verification in a storage case, we have developed a new algorithm. Let's denote the derived tokens as $K$, where $K$ represents the set of derived tokens in a block.

%When derived tokens are added to a block, they are combined with the block number, resulting in the set of derived tokens with block numbers, denoted as $K_{\text{block}}$.
%\[ K_{\text{block}} = \{(k, \text{block\_number}) \mid k \in K\} \]

%The set of derived tokens with block numbers, $K_{\text{block}}$, is then hashed together to create the Merkle root, denoted as $M_{\text{root}}$.
%\[ M_{\text{root}} = \text{hash}(K_{\text{block}}) \]

%The Merkle root, $M_{\text{root}}$, is stored in the block header and the tokenized smart contract.

%When a new block is added, the Merkle root from the previous block, denoted as $M_{\text{prev\_root}}$, is retrieved from the blockchain.

%The new derived tokens in the current block, denoted as $K_{\text{new}}$, are combined with the block index, resulting in the set of derived tokens with block indexes, denoted as $K_{\text{new\_index}}$.
%\[ K_{\text{new\_index}} = \{(k, \text{block\_index}) \mid k \in K_{\text{new}}\} \]

%The Merkle root for the new block, denoted as $M_{\text{new\_root}}$, is computed by hashing the concatenation of $M_{\text{prev\_root}}$, $K_{\text{new\_index}}$, and the block index.
%\[ M_{\text{new\_root}} = \text{hash}(M_{\text{prev\_root}} || K_{\text{new\_index}}) \]

%The resulting Merkle root, $M_{\text{new\_root}}$, represents the combined integrity and traceability of the data dependencies within the blockchain.

%By following this algorithm, we ensure that the derived tokens in each block are combined with block-specific information  and hashed together to create a unique Merkle root. This Merkle root serves as a secure identifier for a case, providing a way to verify data dependencies and ensure the integrity of the provenance records extracted from the storage.

%By following this algorithm, we ensure that the derived tokens in each block are combined with block-specific information (block number and index) and hashed together to create a unique Merkle root. This Merkle root serves as a secure identifier for the block, providing a way to verify data dependencies and ensure the integrity of the blockchain.
%\end{enumerate}

%To verify the versioning of a specific case, any node of the Merkle DAG can be queried on the block headers. The corresponding token transaction containing the list of nodes, including the initial token, can be extracted for validation.

%The use of Merkle roots in the block headers ensures the immutability and integrity of the provenance versioning within the blockchain. Each Merkle root represents a specific aspect of the versioning process, allowing for efficient and secure verification of the transaction history and relationships associated with individual cases.


\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{Sections/Figures/merkle-tree.png}
  \caption{Merkle Tree per each case}
  \label{fig:Merkle-Tree}
\end{figure}










\begin{table}[h]
\centering
\caption{Provenance Records for the ForensiBlock System}
\label{tab:provenance}
\begin{tabular}{|l{3cm}|p{5cm}|}
\hline
\textbf{Record} & \textbf{Description} \\
\hline
Case Number & Unique identifier for a case \\
\hline
Timestamp & Time of the action/event \\
\hline
Initial Block Number & Block where the initial case transaction was recorded \\

\hline
Current Stage & Current stage of the case \\
\hline
Token List & List of tokens associated with the case \\
\hline
Access Request & User request to access specific case data \\
\hline
Client Info & Information about the user/client \\
\hline
Token dependency & analyzed Tokens drived from a files \\
\hline
Validity of Access & Matching system permissions for the access request \\
\hline
Stage Change & Change in the tokenized smart contract's stage \\
\hline
Type of Data Upload & Indicates raw data or analyzed data \\
\hline
\end{tabular}
\end{table}






%The complexity of searching for provenance records on this blockchain design depends on the specific query and the number of transactions and blocks in the blockchain. However, the design incorporates elements that can optimize the search process and make it efficient.

%Searching for a specific case: With the inclusion of the block number of the initial request for each case, the blockchain design knows where to start searching. By leveraging the case numbers associated with transactions, the search can extract and focus on the relevant transactions related to the specified case, reducing the search space and complexity.

%Tracing edits and history: The transactions recorded in the blockchain contain token identifiers and information about the tokens produced from previous edits. This allows for easy traversal of the blockchain and the construction of a hierarchical representation of the edits made to the data over time. By utilizing this hierarchy, the search for provenance records can follow a specific path and track the sequence of edits, simplifying the process and reducing complexity.

%In terms of complexity, searching for provenance records on this blockchain design can be more efficient compared to a backward search. The inclusion of case numbers and token identifiers provides direct references and enables targeted retrieval of relevant information. Instead of scanning the entire blockchain, the search process can be optimized to extract specific transactions and follow the hierarchy of edits, resulting in improved efficiency and reduced complexity.

==> Sections/Discussion.tex <==
Data Tracking: Blockchain enables the creation of a comprehensive and auditable trail of data transactions. Each transaction is recorded as a block, containing a timestamp, transaction details, and a unique identifier. This allows for the transparent tracking of data throughout its lifecycle, from initial upload to subsequent edits.

Data Integrity: The immutability of blockchain ensures that once data is recorded, it cannot be altered or deleted without leaving a trace. This feature is crucial in maintaining the integrity of forensic evidence and preventing unauthorized modifications.

Data Security: Blockchain employs advanced cryptographic techniques to secure data. Transactions are cryptographically hashed and linked to the previous block, forming a chain of blocks. This makes it extremely difficult for malicious actors to tamper with the data stored on the blockchain.

Accountability: The transparent nature of blockchain provides a high level of accountability. Every transaction is associated with a user, and the system records the roles involved in each case. This enhances the accountability of individuals involved in the data handling process.

Trust and Collaboration: By removing the need for a central authority, the proposed system promotes trust and collaboration among multiple stakeholders. It allows authorized users to securely share and access data, facilitating efficient collaboration in forensic investigations.




The framework you described incorporates several security measures to prevent various attacks. Here are some attacks that the framework prevents and the corresponding security measures it employs:

Unauthorized access:

Security measure: The framework uses a registration phase where users are required to register on the blockchain. Only registered users with valid public-private key pairs can participate in subsequent phases, ensuring that unauthorized users cannot access the system.
Data tampering:

Security measure: The framework ensures data integrity by employing cryptographic techniques. Transactions are signed with the sender's private key, and the signature serves as proof of origin and integrity. Any attempt to modify the data will result in an invalid signature, and the tampering will be detected during verification.
Replay attacks:

Security measure: The framework utilizes nonces in requests and transactions. A nonce is a unique token generated for each request, preventing replay attacks. The recipient verifies that the received nonce matches the expected value, ensuring that each request or transaction is processed only once.
Man-in-the-middle attacks:

Security measure: The framework prevents man-in-the-middle attacks by encrypting data, including the nonce and message signatures, within requests and transactions. Encryption ensures that data remains confidential and cannot be intercepted or modified by an attacker during transmission.
Unauthorized stage changes:

Security measure: Only users with specified roles and permissions can trigger stage change transactions. The access control smart contract verifies the user's role and determines whether they have the authority to initiate a stage change. Unauthorized users are denied access, preventing unauthorized stage modifications.
Untrusted data storage:

Security measure: Data uploaded to storage is associated with a token identifier. The storage receives encrypted data and the corresponding token, ensuring that only authorized users with the token can access the data. This prevents unauthorized access to data stored in the system.
Auditing and detection of malicious activity:

Security measure: The framework maintains a log of user requests, transactions, and access results on the blockchain. This logging mechanism allows for auditing and detection of any unauthorized requests or attempts to modify data. By monitoring and analyzing the blockchain's transaction history, malicious activity can be identified and appropriate actions can be taken.
Overall, the framework employs encryption, digital signatures, nonces, access control mechanisms, and blockchain-based logging to ensure data confidentiality, integrity, authentication, and prevention of various attacks. These security measures work together to provide a robust and secure environment for sharing and managing data within the blockchain system.

==> Sections/Implementation.tex <==
\section{Implementation}
\subsection{Blockchain Implementation}

